Expected Validation Performance and Estimation of a Random Variable's Maximum

Research in NLP is often supported by experimental results, and improved reporting of such results can lead to better understanding and more reproducible science. In this paper we analyze three statistical estimators for expected validation performance, a tool used for reporting performance (e.g., accuracy) as a function of computational budget (e.g., number of hyperparameter tuning experiments). Where previous work analyzing such estimators focused on the bias, we also examine the variance and mean squared error (MSE). In both synthetic and realistic scenarios, we evaluate three estimators and find the unbiased estimator has the highest variance, and the estimator with the smallest variance has the largest bias; the estimator with the smallest MSE strikes a balance between bias and variance, displaying a classic bias-variance tradeoff. We use expected validation performance to compare between different models, and analyze how frequently each estimator leads to drawing incorrect conclusions about which of two models performs best. We find that the two biased estimators lead to the fewest incorrect conclusions, which hints at the importance of minimizing variance and MSE.

==> text/04_intuitions.tex <==
\section{Bias-Variance Tradeoff}

These estimators provide a nice illustration of bias-variance tradeoff.
While all three estimators are asymptotically unbiased as $B\to \infty$, with finite $B$ $\Bias{V_n^B}\leq0$ and $\Bias{W_n^B}\leq0$. 
%In both synthetic and real experiments, we find $V_n^B$ and $W_n^B$ both have lower variance than $U_n^B$, as seen in Figure~\ref{fig:synthetic_bias_and_var}.

We can see from Equation~\ref{eq:u_def} that when $i<n$, $\binom{i}{n}=0$ so $P(\maxrv=X_{(i)})=0$. This means that with the assumptions underlying $U_n^B$, the probability of drawing a sample of $n$ points which has a maximum that is smaller than the $n$th order statistic is 0. \jdcomment{another way of saying this is that when $n=B$ the probability of drawing another $B$ points with a maximum that is higher or lower than $X_{(n)}$ is 0.} $V_n^B$ and $W_n^B$ model the probability that another experimenter might run another $B$ trials and \emph{not} see a value as high as $X_\mathit{max}$, but don't attempt to model the probability that one would find a \emph{higher} value (in general, we can't know whether a higher maximum is even possible). Thus, both are ``shrinkage estimators'' as they are biased towards the sample mean (i.e., downwards).
%This bias more greatly affects curves with a larger difference between the single max-found value and the mean, but all $V_n^B$ curves have this bias. 
%If the range of performance values is similar between two curves, the bias affects them similarly, and therefore would be unlikely to change a conclusion as to which model performs best.

%Consider again the case where $n=B$:  as $U_B^B$ is the observed maximum $X_{\mathit{max}}$, it is  sensitive to outliers, while $V_B^B$ is a more robust estimator. \nascomment{is there a proof of that claim?}
%Again, this comes from $V_n^B$ explicitly modeling the probability that a new sample of size $B$ may not include a max as high as $X_\mathit{max}$, which $U_n^B$ does not model.


%Intuitively, as $V_n^B$ models the probability that another experimenter might run another $B$ trials and \emph{not} see a value as high as $X_\mathit{max}$, but doesn't attempt to model the probability that one would find a \emph{higher} value (in general, we can't know whether a higher maximum is even possible), it has a bias towards the sample mean (i.e., downwards).
%\nascomment{I find this confusing, and seemingly contradictory.  we're saying it's biased but it's asymptotically unbiased.  I think maybe what we need to do is qualify that $B$ is finite from the beginning of this paragraph before turning to the infinite $B$ case.  can someone who took a stats class more recently than me take a stab at getting the facts right so this is not confusing?}

%On the other hand, $U_n^B$ is an unbiased estimator \nascomment{again, qualify with ``finite $B$'' or ``even with finite $B$''?}, but, as we will see, it has higher variance in synthetic and realistic experiments.

==> text/97_estimating_variance.tex <==
\section{Estimating Variance}

The above discussion has focused on estimating the expected value (mean) of the maximum of a sequence of i.i.d.~observations.  We now turn to the variance of that maximum (not to be confused with the variance \emph{of the estimators} $V_n^B$
 and $U_n^B$, discussed in the preceding section!).
 An estimate of the variance helps answer the question, ``if we had a budget to run only $n$ trials, how much variation would expect to see in the maximum observed value $X_{\mathit{max}}$?''
\citet{dodge-etal-2019-show} argued for reporting the variance along the EVP curve (means at different values of $n$).

\nascomment{reworked a lot here, please check}

The conventional method for estimating variance requires a plug-in estimate of the mean; what are the implications of choosing $V_n^B$ or $U_n^B$ as the mean estimate to plug in?
In the finite $B$ case that is relevant here, the differences are stark.

At $n=1$, $V_n^B$ and $U_n^B$ return the sample mean of the $B$ observations, and the resulting sample variance estimate will be the variance of the $B$ observations.  As $n \rightarrow B$, however, the estimated variance for $U_n^B$ goes to zero.  
%When $n=1$, it is the sample variance of the $B$ points, but as $n\to B$ it drops to zero for $U_n^B$ while $V_n^B$ again models the variance from the possibility of resampling $B$ points and finding a max lower than $X_\mathit{max}$.
%Without information about the true distribution it's difficult to model the event that resampling $B$ points would lead to a higher max, and thus we recommend reporting this estimate of variance.
The estimated variance for $V_n^B$ captures the possibility of finding a maximum less than $X_{\mathit{max}}$ (but not a greater one).\footnote{For many distributions this is an underestimate of the true variance \nascomment{this statement is not precise; are we saying this is a biased estimate of variance?  isn't that true for the $U$ version as well though?  the scope of attachment for this footnote is ambiguous}, so computing confidence intervals would likely not contain the quantity of interest appropriately, as shown by \citet{tang-etal-2020-showing}.}
\nascomment{I took out the recommendation here; save that for the end!}

%This difference again comes from the modeling assumption for $V_n^B$ that it's possible to resample $B$ points and find a max lower than $X_\mathit{max}$, which $U_n^B$ does not model.

%With $U_n^B$, as $n\to B$ the variance of the sample mean drops to zero (as there is only one subset of size $B$, the variance is zero).
The modeling assumptions in $U_n^B$ cause the sample variance to go to 0, which could problematically suggest to a reader that if they were to run another set of $B$ experiments, they would find $U_n^B$ to be perfectly stable as $n\to B$.
However, as we will see in the next section, the $U_n^B$ estimator has higher variance (and thus is less stable) than $V_n^B$. 
%We argue that for these reasons, $V_n^B$ leads to more reproducible research.


%$V_n^B$ still has non-zero variance for the sample mean. 
%The sample variance from $U_n^B$'s modeling assumption going to 0 could problematically suggest that if another practitioner were to run another set of $B$ experiments, they would find the same result. $V_n^B$ still has non-zero variance for the sample mean. 

%As we show that $U_n^B$ can have higher variance, but it's estimate of sample variance 
%This suggests---problematically in our view---that if another practitioner were to 





%All else equal, lower variance of a statistical estimator is better. As a further benefit, $U_n^B$'s connection to the bootstrap provides 

%A further benefit 
%Further, with $U_n^B$, as $n\to B$ the variance of the sample mean drops to zero (as there is only one subset of size $B$, the variance is zero). 
%\resolved{\dallas{I think the preceding is too confusing. What we really care about is the variance of the estimator, which is higher for the unbiased one (I think). Here you are saying that it has zero variance, which might confuse people. I'm pretty sure you mean that it will give the same estimate for a given sample, but as written, I'm pretty sure that applies to both estimators (i.e. there is no subsampling; you care considering all sets/subsets), so I'm not sure why it's relevant. }}
%This suggests---problematically in our view---that if another practitioner were to run another set of $B$ experiments, they would find the same result. $V_n^B$ still has non-zero variance for the sample mean. 
%\resolved{\dallas{Maybe I don't understand what you mean by this? I don't see how it's different... If you mean the subsampling thing, I think that's still misleading because it massively underestimates the true variance.}}

